UEOF: A Benchmark Dataset for Underwater Event-Based Optical Flow

Underwater imaging is fundamentally challenging due to wavelength-dependent light attenuation, strong scattering from suspended particles, turbidity-induced blur, and non-uniform illumination. These effects impair standard cameras and make ground-truth motion nearly impossible to obtain. On the other hand, event cameras offer microsecond resolution and high dynamic range. Nonetheless, progress on investigating event cameras for underwater environments has been limited due to the lack of datasets that pair realistic underwater optics with accurate optical flow. To address this problem, we introduce the first synthetic underwater benchmark dataset for event-based optical flow derived from physically-based ray-traced RGBD sequences. Using a modern video-to-event pipeline applied to rendered underwater videos, we produce realistic event data streams with dense ground-truth flow, depth, and camera motion. Moreover, we benchmark state-of-the-art learning-based and model-based optical flow prediction methods to understand how underwater light transport affects event formation and motion estimation accuracy. Our dataset establishes a new baseline for future development and evaluation of underwater event-based perception algorithms. The source code and dataset for this project are publicly available at https://robotic-vision-lab.github.io/ueof.

==> figures/optical_flow_statistics.tex <==
\begin{figure}[h]
    \centering 
    \begin{subfigure}{0.44\linewidth}
      \includegraphics[width=\linewidth,cfbox=gray 0pt 0pt]{images/optical_flow_stats/stats_magnitude_helvetica}
      \caption{Magnitude distribution}
      \label{subfig:optical_flow_magnitude}
      \end{subfigure}
      %
    \begin{subfigure}{0.44\linewidth}
      \includegraphics[width=\linewidth,cfbox=gray 0pt 0pt]{images/optical_flow_stats/stats_uv_helvetica}      \includegraphics[width=0.3\linewidth,cfbox=gray 0pt 0pt]{images/optical_flow_stats/colorbar_legend}
      
      \caption{Pixel displacement}
      \label{subfig:optical_flow_displacement}
    \end{subfigure}
    \caption{Optical flow statistics for the UEOF dataset: (a) the semi-log
    histogram of flow magnitudes indicates a wide dynamic range, with a mean of
    6.1\,px and a significant tail representing fast motion; (b) the joint
    distribution of horizontal ($u$) and vertical ($v$) displacements shows a dense
    coverage of motion directions.}
    \label{fig:optical_flow_statistics}
\end{figure}

==> tables/LOFUE_ANPE.tex <==
\begin{table}
  \centering
  \small
  \resizebox{0.5\textwidth}{!}{
  \begin{tabular}{c l r r r r r}
    \toprule
    \bfseries Method
      & \bfseries Model
      & {\bfseries Scene~1}
      & {\bfseries Scene~2}
      & {\bfseries Scene~3}
      & {\bfseries Scene~4}
      & {\bfseries Scene~5} \\
    \midrule

    % --- SL Group ---
    % \rotatebox[origin=c]{90}{SL}
    \multirow{2}{*}{\rotatebox[origin=c]{90}{LB}}
      & E-RAFT~\cite{gehrig2021eraft}
      & \makecell[r]{\textbf{59.24} \\ \underline{47.72} \\ \underline{42.30} \\ \underline{36.10} \\ 26.52 \\ 9.43}
      & \makecell[r]{97.9 \\ 92.7 \\ 85.1 \\ 66.8 \\ 23.5 \\ 4.00}
      & \makecell[r]{90.64 \\ 72.78 \\ 57.19 \\ 42.11 \\ 20.20 \\ 10.23}
      & \makecell[r]{96.26 \\ 91.34 \\ 85.62 \\ 68.21 \\ 19.78 \\ 4.16}
      & \makecell[r]{\textbf{43.85} \\ \underline{36.71} \\ 33.70 \\ 29.71 \\ 23.52 \\ 20.07} \\
    
    % \midrule 
    
    % --- USL Group ---
    % \rotatebox[origin=c]{90}{USL}
      & MotionPriorCMax~\cite{hamann2024motionprior}
      & \makecell[r]{83.13 \\ \textbf{30.53} \\ \textbf{21.38} \\ \textbf{12.62} \\ \textbf{3.61} \\ 1.2}
      & \makecell[r]{56.16 \\ 18.28 \\ \underline{8.10} \\ \textbf{3.25} \\ \underline{1.06} \\ 0.17}
      & \makecell[r]{72.1 \\ 24.2 \\ \textbf{11.53} \\ \textbf{5.19} \\ \underline{1.47} \\ \underline{0.25}}
      & \makecell[r]{65.52 \\ 15.67 \\ \textbf{5.13} \\ \textbf{2.25} \\ \underline{0.37} \\ \textbf{0.02}}
      & \makecell[r]{83.09 \\ \textbf{20.60} \\ \textbf{13.76} \\ \textbf{0.982} \\ \textbf{0.347} \\ \underline{0.24}} \\
    
    \midrule 
    
    % --- MB Group ---
    \multirow{3}{*}{\rotatebox[origin=c]{90}{MB}}
      & EINCM~\cite{karmokar2025secrets}
      & \makecell[r]{\underline{69.50} \\ 63.22 \\ 59.93 \\ 50.28 \\ 5.57 \\ \underline{0.014}}
      & \makecell[r]{44.34 \\ 26.674 \\ 20.3957 \\ 13.6578 \\ 8.416 \\ 7.007}
      & \makecell[r]{\underline{27.413} \\ \underline{18.739} \\ 14.8810 \\ 10.5998 \\ 6.1993 \\ 1.6001}
      & \makecell[r]{\underline{18.8756} \\ \underline{8.9175} \\ 6.2236 \\ 3.7885 \\ 1.096 \\ 0.2980}
      & \makecell[r]{75.6051 \\ 66.2166 \\ 58.8357 \\ 35.9175 \\ 4.1083 \\ 0.8785} \\
      
    
      & MultiCM~\cite{shiba2022secrets}
      & \makecell[r]{75.11 \\ 73.59 \\ 71.19 \\ 61.17 \\ \underline{5.54} \\ \textbf{0.0019}}
      & \makecell[r]{\underline{41.96} \\ \textbf{12.66} \\ \textbf{6.91} \\ 3.97 \\ 1.33 \\ 0.306}
      & \makecell[r]{59.56 \\ 35.00 \\ 23.31 \\ 12.52 \\ 3.42 \\ 0.539}
      & \makecell[r]{41.39 \\ 18.27 \\ 9.23 \\ 3.80 \\ 0.578 \\ 0.202}
      & \makecell[r]{\underline{69.33} \\ 40.26 \\ \underline{23.54} \\ \underline{10.00} \\ \underline{1.50} \\ \textbf{0.0837}} \\

    % \midrule
      % -- multi modal

      % \multirow{2}{*}{\rotatebox[origin=c]{90}{\scriptsize Multi-Modal}}
      & OPCM~\cite{karmokar2025inertia}
      & \makecell[r]{ \\  \\  \\ \\  \\ }
      & \makecell[r]{58.4687 \\ 25.1368 \\ 11.1714 \\ \underline{3.3275} \\ \textbf{0.6028} \\ \textbf{0.0008}} 
      & \makecell[r]{72.7975 \\ 33.4511 \\ 19.6623 \\ \underline{8.2933} \\ \textbf{1.1730} \\ \textbf{0.0499}} 
      & \makecell[r]{80.4583 \\ 37.4519 \\ 12.7480 \\ \underline{2.4106} \\ \textbf{0.2535} \\ \underline{0.0528}} 
      & \makecell[r]{ \\  \\  \\ \\  \\ } \\
      
    % \addlinespace 
    
    %   & Multi-Modal EINCM ~\cite{}
    %   & \makecell[r]{ \\  \\  \\ \\  \\ } 
    %   & \makecell[r]{\textbf{32.6391} \\ \underline{13.7557} \\ 8.3787 \\ 3.9107 \\ 1.0714 \\ \underline{0.1403}}
    %   & \makecell[r]{\textbf{26.6571} \\ \textbf{18.0729} \\ \underline{14.2461} \\ 10.0540 \\ 5.7540 \\ 1.3929} 
    %   & \makecell[r]{\textbf{18.8010} \\ \textbf{8.8445} \\ \underline{6.1526} \\ 3.6931 \\ 0.9301 \\ 0.2625} 
    %   & \makecell[r]{ \\  \\  \\ \\  \\ } \\

    %   \addlinespace

    \bottomrule
  \end{tabular}
  \caption{The N-pixel error rates on the UEOF dataset (shallow-water
  environment) across five scenes at $dt=1$. \textbf{Bold} indicates best,
  \underline{underline} indicates second-best.}
  \label{tab:ferone_anpe}
  }
\end{table}

==> tables/LOFUE_ANPE_horizontal.tex <==
\begin{table*}%[ht]
    \centering
    
    \begin{adjustbox}{max width=\textwidth}
    \begin{tabular}{%
        @{}c@{\thickspace}l 
        c c c c c c
        c c c c c c
        c c c c c c%
    }
        \toprule
        % \bfseries Method
        {}
        & Model
        & \multicolumn{6}{c}{Scene~1}
        & \multicolumn{6}{c}{Scene~2}
        & \multicolumn{6}{c}{Scene~3}\\
        
        \cmidrule(lr){3-8} \cmidrule(lr){9-14} \cmidrule(lr){15-20} 
        
        {} & {}
        % scene1
        & A1PE ($\downarrow$)
        & A2PE ($\downarrow$)
        & A3PE ($\downarrow$)
        & A5PE ($\downarrow$)
        & A10PE ($\downarrow$)
        & A20PE ($\downarrow$)
        % scene2
        & A1PE ($\downarrow$)
        & A2PE ($\downarrow$)
        & A3PE ($\downarrow$)
        & A5PE ($\downarrow$)
        & A10PE ($\downarrow$)
        & A20PE ($\downarrow$)
        % scene3
        & A1PE ($\downarrow$)
        & A2PE ($\downarrow$)
        & A3PE ($\downarrow$)
        & A5PE ($\downarrow$)
        & A10PE ($\downarrow$)
        & A20PE ($\downarrow$)\\
        
        \midrule
        
        % --- LB Group ---
        \multirow{2}{*}{\rotatebox[origin=c]{90}{LB}}
        & E-RAFT~\cite{gehrig2021eraft}
        % scene1
        & \textbf{59.24} & \underline{47.72} & \underline{42.30} & \underline{36.10} & 26.52 & 9.43
        % scene2
        & 97.9           & 92.7              & 85.1              & 66.8              & 23.5  & 4.00
        % scene3
        & 90.64          & 72.78             & 57.19             & 42.11             & 20.20 & 10.23\\
        
        & MotionPriorCMax~\cite{hamann2024motionprior}
        % scene1
        & 83.13 & \textbf{30.53} & \textbf{21.38}   & \textbf{12.62} & \textbf{3.61}    & 1.2
        % scene2
        & 56.16 & 18.28          & \underline{8.10} & \textbf{3.25}  & \underline{1.06} & 0.17
        % scene3
        & 72.1  & 24.2           & \textbf{11.53}   & \textbf{5.19}  & \underline{1.47} & \underline{0.25}\\
        
        \midrule 
        
        % --- MB Group ---
        \multirow{3}{*}{\rotatebox[origin=c]{90}{MB}}
        & EINCM~\cite{karmokar2025secrets}
        % scene1
        & \underline{69.50}  & 63.22              & 59.93   & 50.28   & 5.57  & \underline{0.014}
        % scene2
        & 44.34              & 26.67             & 20.40 & 13.66 & 8.42 & 7.01
        % scene3
        & \underline{27.41} & \underline{18.74} & 14.88 & 10.60 & 6.20 & 1.60\\
        
        & MultiCM~\cite{shiba2022secrets}
        % scene1
        & 75.11             & 73.59          & 71.19         & 61.17 & \underline{5.54} & \textbf{0.0019}
        % scene2
        & \underline{41.96} & \textbf{12.66} & \textbf{6.91} & 3.97  & 1.33             & 0.31
        % scene3
        & 59.56             & 35.00          & 23.31         & 12.52 & 3.42             & 0.54\\

        & OPCM~\cite{karmokar2026orientation}
        % scene1
        & {}      & {}      & {}      & {}                 & {}              & {}
        % scene2
        & 58.47 & 25.14 & 11.17 & \underline{3.33} & \textbf{0.60} & \textbf{0.0008}
        % scene3
        & 72.80 & 33.45 & 19.66 & \underline{8.29} & \textbf{1.17} & \textbf{0.05}\\
        
        
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

        \toprule
        % \bfseries Method
        {}
        & {}
        & \multicolumn{6}{c}{Scene~4}
        & \multicolumn{6}{c}{Scene~5}
        & \multicolumn{6}{c}{}\\
        
        \cmidrule(lr){3-8} \cmidrule(lr){9-14}
        
        {} & {}
        % scene4
        & A1PE ($\downarrow$)
        & A2PE ($\downarrow$)
        & A3PE ($\downarrow$)
        & A5PE ($\downarrow$)
        & A10PE ($\downarrow$)
        & A20PE ($\downarrow$)
        % scene5
        & A1PE ($\downarrow$)
        & A2PE ($\downarrow$)
        & A3PE ($\downarrow$)
        & A5PE ($\downarrow$)
        & A10PE ($\downarrow$)
        & A20PE ($\downarrow$)
        % 
        & {} 
        & {} 
        & {} 
        & {} 
        & {} 
        & {} \\
        
        \midrule
        
        % --- SL Group ---
        % \rotatebox[origin=c]{90}{SL}
        \multirow{2}{*}{\rotatebox[origin=c]{90}{LB}}
        & E-RAFT~\cite{gehrig2021eraft}
        % scene4
        & 96.26          & 91.34             & 85.62             & 68.21             & 19.78 & 4.16
        % scene5
        & \textbf{43.85} & \underline{36.71} & 33.70             & 29.71             & 23.52 & 20.07 
        % 
        & {}             & {}                & {}                & {}                & {}    & {} \\
        
        % \midrule 
        
        % --- USL Group ---
        % \rotatebox[origin=c]{90}{USL}
        & MotionPriorCMax~\cite{hamann2024motionprior}
        % scene4
        & 65.52 & 15.67          & \textbf{5.13}    & \textbf{2.25}  & \underline{0.37} & \textbf{0.02}
        % scene5
        & 83.09 & \textbf{20.60} & \textbf{13.76}   & \textbf{0.98} & \textbf{0.35}   & \underline{0.24}
        % 
        & {}    & {}             & {}               & {}              & {}              & {} \\
        
        \midrule 
        
        % --- MB Group ---
        \multirow{3}{*}{\rotatebox[origin=c]{90}{MB}}
        & EINCM~\cite{karmokar2025inertia}
        % scene4
        & \underline{18.88} & \underline{8.92} & 6.22  & 3.79  & 1.10  & 0.30
        % scene5
        & 75.61             & 66.22            & 58.84 & 35.92 & 4.11 & 0.88 
        % 
        & {}                  & {}                 & {}      & {}      & {}     & {} \\
        
        
        & MultiCM~\cite{shiba2022secrets}
        % scene4
        & 41.39             & 18.27 & 9.23              & 3.80              & 0.58            & 0.20
        % scene5
        & \underline{69.33} & 40.26 & \underline{23.54} & \underline{10.00} & \underline{1.50} & \textbf{0.084}
        % 
        & {}                & {}    & {}                & {}                & {}               & {} \\
        
        % \midrule
        % -- multi modal
        
        % \multirow{2}{*}{\rotatebox[origin=c]{90}{\scriptsize Multi-Modal}}
        & OPCM~\cite{karmokar2025inertia}
        % scene4
        & 80.46 & 37.45 & 12.75 & \underline{2.41} & \textbf{0.25} & \underline{0.053}
        % scene5
        &         &         &         &                    &                 & 
        % 
        & {}      & {}      & {}      & {}                 & {}              & {} \\
        
          
        % \addlinespace 
        
        %   & Multi-Modal EINCM ~\cite{}
        %   & \makecell[r]{ \\  \\  \\ \\  \\ } 
        %   & \makecell[r]{\textbf{32.6391} \\ \underline{13.7557} \\ 8.3787 \\ 3.9107 \\ 1.0714 \\ \underline{0.1403}}
        %   & \makecell[r]{\textbf{26.6571} \\ \textbf{18.0729} \\ \underline{14.2461} \\ 10.0540 \\ 5.7540 \\ 1.3929} 
        %   & \makecell[r]{\textbf{18.8010} \\ \textbf{8.8445} \\ \underline{6.1526} \\ 3.6931 \\ 0.9301 \\ 0.2625} 
        %   & \makecell[r]{ \\  \\  \\ \\  \\ } \\
        
        %   \addlinespace
        
        \bottomrule
    \end{tabular}
    \end{adjustbox}
    \caption{N-pixel error rates on the UEOF dataset (shallow-water environment)
    across five scenes at $dt = 1$. In each cell: A1PE, A2PE, A3PE, A5PE, A10PE,
    A20PE. \textbf{Bold} indicates best, \underline{underline} indicates
    second-best.}
    \label{tab:lofue_anpe}
\end{table*}

==> tables/VAROS_ANPE.tex <==
\begin{table}
  \centering
  \small
  \caption{The N-pixel error rates on the VAROS Dataset across five scenes at
  $dt=1$. \textbf{Bold} indicates best, \underline{underline} indicates
  second-best.}
  \label{tab:varos_npe_old}
  \begin{tabularx}{\textwidth}{c l *{5}{R}}
    \toprule
    \bfseries Method
      & \bfseries Model
      & {\bfseries Scene~1}
      & {\bfseries Scene~2}
      & {\bfseries Scene~3}
      & {\bfseries Scene~4}
      & {\bfseries Scene~5} \\
    \midrule

    % --- SL Group (1 model) ---
    \rotatebox[origin=c]{90}{SL}
      & E-RAFT~\cite{gehrig2021eraft}
      & \makecell[r]{72.43 \\ 51.13 \\ 38.96 \\ 23.72 \\ 8.63 \\ 4.13}
      & \makecell[r]{98.37 \\ 94.41 \\ 89.66 \\ 77.83 \\ 42.58 \\ 5.92}
      & \makecell[r]{59.61 \\ 41.97 \\ 31.88 \\ 19.44 \\ 7.96 \\ 3.13}
      & \makecell[r]{69.48 \\ 53.99 \\ 47.92 \\ 40.25 \\ 16.08 \\ 4.06}
      & \makecell[r]{65.11 \\ 45.71 \\ 33.23 \\ 20.13 \\ 7.09 \\ 1.34} \\

    \midrule

    % --- USL Group (1 model) ---
    \rotatebox[origin=c]{90}{USL}
      & MotionPriorCMax~\cite{hamann2024motionprior}
      & \makecell[r]{92.70 \\ 81.71 \\ 69.04 \\ 47.35 \\ 21.45 \\ 5.65}
      & \makecell[r]{84.83 \\ 70.28 \\ 59.20 \\ 42.94 \\ 16.66 \\ 2.20}
      & \makecell[r]{85.97 \\ 70.72 \\ 59.64 \\ 42.71 \\ 18.86 \\ 4.94}
      & \makecell[r]{87.87 \\ 78.54 \\ 72.07 \\ 60.35 \\ 26.36 \\ 3.35}
      & \makecell[r]{85.94 \\ 71.70 \\ 59.70 \\ 37.66 \\ 13.29 \\ 2.11} \\

    \midrule

    % --- MB Group (2 models) ---
    \multirow{2}{*}{\rotatebox[origin=c]{90}{MB}}
      & EINCM~\cite{karmokar2025secrets}
      & \makecell[r]{60.92 \\ 47.67 \\ 38.76 \\ 25.58 \\ 10.44 \\ 2.95}
      & \makecell[r]{41.39 \\ 30.39 \\ 24.40 \\ 16.72 \\ 6.75 \\ 1.07}
      & \makecell[r]{50.15 \\ 37.40 \\ 30.55 \\ 23.10 \\ 12.85 \\ 3.25}
      & \makecell[r]{37.46 \\ 26.61 \\ 20.38 \\ 12.54 \\ 4.97 \\ 1.57 \\ 0.14}
      & \makecell[r]{47.20 \\ 31.50 \\ 23.80 \\ 15.90 \\ 6.45 \\ 0.95} \\

    \addlinespace

      & MultiCM~\cite{shiba2022secrets}
      & \makecell[r]{60.38 \\ 44.94 \\ 36.86 \\ 27.62 \\ 13.81 \\ 4.34}
      & \makecell[r]{47.33 \\ 33.10 \\ 24.67 \\ 14.48 \\ 4.52 \\ 0.598}
      & \makecell[r]{48.66 \\ 36.03 \\ 29.19 \\ 21.29 \\ 10.73 \\ 2.12}
      & \makecell[r]{39.79 \\ 25.98 \\ 18.83 \\ 11.68 \\ 4.88 \\ 0.536}
      & \makecell[r]{45.87 \\ 30.02 \\ 22.44 \\ 14.06 \\ 5.28 \\ 0.509} \\

    \bottomrule
  \end{tabularx}
\end{table}

==> tables/dataset_comparison.tex <==
% --------------------------------------------------------------------------------
\begin{table}
    \centering
    
    \begin{adjustbox}{max width=\linewidth}
    % -------------------------------------------------------------------------
    % Table Content
    % -------------------------------------------------------------------------
    % Adjusted to 8 columns (removed 2nd column 'c')
    \begin{tabular}{l l c c c c c c}
        \toprule
        % Top Header structure
        % Shifted Scale to col 4, Modalities to cols 5-8
        & & & \multicolumn{1}{c}{{Scale}} & \multicolumn{4}{c}{{Modalities}} \\
        \cmidrule(lr){4-4} \cmidrule(lr){5-8}

        % Column Headers
        {Dataset} & 
        {Sensor / Sim.} & {Res ($W \times H$)} & 
        {Duration} & {RGB} & {Events} & {Flow} & {Vel} \\
        \midrule

        % ---------------------------------------------------------------------
        % Real-World Datasets
        % ---------------------------------------------------------------------
        % Adjusted multicolumn width to 8
        \multicolumn{8}{l}{\textit{Real-World Datasets}} \\
        \midrule
        
        AquaticVision \cite{peng2025aquaticvision} & 
        DAVIS346 & $346 \times 260$ &
        13m06s & \xmark & \cmark & \xmark & \cmark \\
        
        OsloMet \cite{saksvik2023oslomet} & 
        DAVIS346 & $346 \times 260$ &
        -      & \xmark & \cmark & \xmark & \cmark \\
        
        Aqua-eye/UWTB \cite{luo2023transcodnet,guo2025utnet} & 
        DAVIS346 & $346 \times 260$ &
        -      & \xmark & \cmark & \xmark & \xmark \\
        
        DAVIS-NUIUIED \cite{bi2022non} & 
        DAVIS346 & $346 \times 260$ &
        -      & \cmark & \cmark & \xmark & \xmark \\

        \midrule
        % ---------------------------------------------------------------------
        % Synthetic and Converted Datasets
        % ---------------------------------------------------------------------
        \multicolumn{8}{l}{\textit{Synthetic and Converted Datasets}} \\
        \midrule
        
        EvtSlowTV \cite{macaulay2025evtslowtv} & 
        YouTube$\rightarrow$ESIM & Var.               & 
        -    & \cmark & \cmark & \xmark & \xmark \\
        
        eStonefish \cite{mansour2025estonefish} & 
        Stonefish                & $1280 \times 720$  & 
        6m & \xmark & \cmark & \cmark & \xmark \\
        
        EREBUS \cite{kyatham2025erebus} & 
        Blender$\rightarrow$V2E  & $1920 \times 1080$ & 
        -   & \cmark & \cmark & \xmark & \xmark \\

        % ---------------------------------------------------------------------
        % Ours
        % ---------------------------------------------------------------------
        \rowcolor{gray!10} 
        {UEOF (ours)} & 
        {Blender$\rightarrow$V2E} & ${1280 \times 720}^{\ast}$ & 
        {12m51s} & {\cmark} & {\cmark} & {\cmark} & {\cmark} \\
        
        \bottomrule
    \end{tabular}
    \end{adjustbox}
    % -------------------------------------------------------------------------
    % Footnotes
    % -------------------------------------------------------------------------
    \vspace{-2mm} 
    \begin{minipage}{0.95\linewidth}
        \tiny 
        $^{\ast}$ Includes subsets at $960 \times 540$. 
    \end{minipage}
    % \vspace{-4mm}
    \caption{A comparison of existing underwater event-based datasets. Our UEOF
    dataset is complete with RGB/event data as well as ground-truth optical flow
    and ego-velocities. \textit{Duration}: Total recording duration. \textit{Vel}:
    Camera Ego-Velocity. \textit{Flow}: Optical Flow. \add{Need to update caption}}
    \label{tab:dataset_comparison}
\end{table}
